ReMoDiffuse: Retrieval-Augmented Motion Diffusion Model

3D human motion generation is crucial for creative industry. Recent advances rely on generative models with domain knowledge for text-driven motion generation, leading to substantial progress in capturing common motions. However, the performance on more diverse motions remains unsatisfactory. In this work, we propose ReMoDiffuse, a diffusion-model-based motion generation framework that integrates a retrieval mechanism to refine the denoising process. ReMoDiffuse enhances the generalizability and diversity of text-driven motion generation with three key designs: 1) Hybrid Retrieval finds appropriate references from the database in terms of both semantic and kinematic similarities. 2) Semantic-Modulated Transformer selectively absorbs retrieval knowledge, adapting to the difference between retrieved samples and the target motion sequence. 3) Condition Mixture better utilizes the retrieval database during inference, overcoming the scale sensitivity in classifier-free guidance. Extensive experiments demonstrate that ReMoDiffuse outperforms state-of-the-art methods by balancing both text-motion consistency and motion quality, especially for more diverse motion generation.

==> sections/supp_00_implementation.tex <==
\section{Implementation Detail}



\begin{figure}[]
    \centering
    \includegraphics[width=\linewidth]{figures/stylization.png}
    \caption{\textbf{Architecture} of the stylization block. This module is adapted from MotionDiffuse~\cite{zhang2022motiondiffuse}. We remove the prompt embedding from the original design to better support classifier-free guidance. This module attempts to inject the information of the current timestamp into the feature representation, which is necessary for denoising steps. Specifically, the timestamp embedding $e_t$ is fed into a series of transformation layers. Two embeddings are generated afterward and serve as an additive offset and a multiplicative offset to the original feature map, respectively. }
    \label{fig:style}
    \vspace{-10pt}
\end{figure}


\subsection{Stylization Block}

Similar to MotionDiffuse~\cite{zhang2022motiondiffuse} and MDM~\cite{tevet2022human}, we build up our pipeline on the basis of transformer layers. In both semantics-modulated attention modules and FFN modules, following MotionDiffuse~\cite{zhang2022motiondiffuse}, we add a stylization block to fuse timestamp $t$ into the motion generation process. First, an embedding vector $\mathbf{e_t}$ is obtained from the timestamp $t$. Then for each block, a residual shortcut is applied between the input $\mathbf{X} \in \mathbb{R}^{n \times d}$ and the output $\mathbf{Y} \in \mathbb{R}^{n \times d}$, where $n$ is the number of elements and $d$ is the dimensionality. The detailed structure is shown in Figure ~\ref{fig:style}.

\subsection{Condition Mixture}


\noindent\paragraph{Constrastive Model.} To imitate the evaluator used in the standard evaluation process, we train our contrastive model, which aims at encoding the paired text descriptions and motion sequences into a joint embedding space. As for the motion encoder, we use a 4-layer ACTOR~\cite{petrovich2021action} Encoder. The text encoder is identical to the one we used in \name. The only difference is that we require a sentence feature instead of a sequence of word features. We train this contrastive learning model with the same loss in Guo \etal ~\cite{guo2022generating}. 20K and 40K optimization steps are applied for the KIT-ML and HumanML3D datasets, respectively. Table ~\ref{tab:evaluator} shows the evaluation results of the real motions.

\begin{table*}[ht]
\centering
\caption{\textbf{Evaluation results of different evaluator.}}
\label{tab:evaluator}
\setlength{\tabcolsep}{1.4mm}
{
\begin{tabular}{lcccccccc}
\hline
\multirow{2}{2cm}{\centering Methods} & \multirow{2}{2cm}{\centering Dataset} & \multicolumn{3}{c}{\centering R Precision$\uparrow$} & \multirow{2}{1.5cm}{\centering FID$\downarrow$} & \multirow{2}{2.5cm}{\centering MM Dist$\downarrow$} & \multirow{2}{2cm}{\centering Diversity$\uparrow$} \\
& &  Top 1 & Top 2 & Top 3 \\
\hline
Guo \etal & HumanML3D & $0.511^{\pm .003}$ & $0.703^{\pm.003}$ & $0.797^{\pm.002}$ & $0.002^{\pm.000}$ & $2.974^{\pm.008}$ & $9.503^{\pm.065}$ \\
Ours & HumanML3D & $0.539^{\pm .004}$ & $0.721^{\pm.003}$ & $0.810^{\pm.003}$ & $0.001^{\pm.000}$ & $1.462^{\pm.006}$ & $5.298^{\pm.047}$ \\
\hline
Guo \etal & KIT-ML & $0.424^{\pm .005}$ & $0.649^{\pm.006}$ & $0.779^{\pm.006}$ & $0.031^{\pm.004}$ & $2.788^{\pm.012}$ & $11.08^{\pm.097}$ \\ 
Ours & KIT-ML & $0.475^{\pm .006}$ & $0.690^{\pm.004}$ & $0.791^{\pm.005}$ & $0.002^{\pm.000}$ & $1.337^{\pm.012}$ & $6.371^{\pm.058}$ \\
\hline
\end{tabular}}
\end{table*}


\begin{table*}[ht]
\centering
\caption{\textbf{Examples of Rareness in the HumanML3D test set.}}
\label{tab:example}
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{1.4mm}
{
\begin{tabular}{ccp{12cm}}
\hline

\textbf{Rareness} & \textbf{Rareness Quantile} & \textbf{Caption} \\
\hline
$0.0000$ & $0.00\%$ & \textit{a person slowly jumped forward} \\ 
$0.0110$ & $9.89\%$ & \textit{a man walks counterclockwise in a circle} \\
$0.0283$ & $22.09\%$ & \textit{the person quickly walks forward, and picks something up.} \\
$0.0361$ & $31.49\%$ & \textit{a person picks an item up and moves it a foot to their right and places it down.} \\
$0.0442$ & $44.96\%$ & \textit{a man sidesteps suddenly to his left, bumps into something and leans over, looks around, then walks to his left, bumping into something else and once more leaning over.} \\
$0.0502$ & $55.07\%$ & \textit{someone walks with difficulty on their right side, then tries to run} \\
% $0.0616$ & $71.70\%$ & \textit{a person stretches their hips, then arms, then bends forwards and steps forwards.} \\
$0.0784$ & $86.40\%$ & \textit{a person takes in big steps in a hurry walking into the rectangular area while hands are dangling and swinging.} \\
$0.0866$ & $90.87\%$ & \textit{someone puts both of their hands on their chests and appears to be laughing. then waves their left hand.} \\
$0.1051$ & $96.04\%$ & \textit{a person crosses his arms in an x-shape out in front of him and then quickly swings them to the side, brushes off is left leg with his left hand, and then raises his left hand as if to wave.} \\
$0.1872$ & $99.78\%$ & \textit{a person makes several hand gestures and appears to move objects around.} \\
\hline

\end{tabular}}
\end{table*}

\noindent\paragraph{Parameter Finetuning.} As mentioned before, we only use 50 denoising steps to generate motion sequences in the inference stage. However, it is impractical to calculate the gradient through such several forward times. To simplify the problem, we divide all denoising steps into the first 40 steps and the last ten steps. In the first part, we use grid search to find a better parameter combination. Specifically, as for the output formulation:
\begin{equation}
\label{eq:result}
\begin{aligned}
\widehat{S} =& w_1 \cdot S(\mathbf{x}_t,t,\mathrm{retr}, \mathrm{text}) + w_2 \cdot S(\mathbf{x}_t,t,\mathrm{text}) + \\
            & w_3 \cdot S(\mathbf{x}_t,t,\mathrm{retr}) + w_4 \cdot S(\mathbf{x}_t,t),
\end{aligned}
\end{equation}
We search $w_1$ and $w_2$ from $[-5, 5]$ with step $0.5$ to find the best parameter for each model. Here we use inspiration from Re-Imagen~\cite{chen2022re} that set $w_4=0$. Besides, to retain the output's statistics, we $w_1 + w_2 + w_3 + w_4=1$. These two properties enable us to find the optimal combination by only searching the value of $w_1$ and $w_2$. The evaluation metric is the calculated FID between our generated sequences and the natural motion sequences in the training split performed by our trained contrastive model. This search aims to find an optimal combination of $w_1$ and $w_2$ to achieve the lowest FID.

In the second stage, we use an end-to-end training scheme to optimize $w_1, w_2$, and $w_3$. $w_4$ is acquired by $1-w_1-w_2-w_3$. We use the Adam optimizer to train our model on the training split for 1K steps to find the best parameter combination.

We use the searched parameters during training to perform the first 40 denoising steps. After that, we auto-regressively denoise the motion sequence with learnable $w_1, w_2$ and $w_3$. The training objective here is also reducing FID.

We use the Adam optimizer and train 1K steps for both HumanML3D and KIT-ML datasets to find the best parameter combination.

==> sections/supp_01_imbalance.tex <==
\section{Data Analysis}





In the main text, we define the rareness $r_p$ as:
\begin{equation}
    r_p = 1 - \max\limits_i \{<E_T(t_i), E_T(\mathrm{prompt})>\},
\end{equation}
where $E_T$ denotes the text encoder in the CLIP~\cite{radford2021learning} model, $t_i$ is the motion description in the training set, and $<\cdot, \cdot>$ represents the cosine similarity of the two given vectors. Intuitively, this formulation measures the maximum similarity between the given prompt and training prompts. The rareness will be lower if this similarity is larger, and vice versa.

Figure ~\ref{fig:dist} shows the distribution of rareness. The minimum value is almost 0, meaning some captions in the test split are similar to some of the training split. The maximum value is less than 0.25. We divide the whole distribution into 100 bins as the requirement of our proposed \textit{balanced MM}. Most test data concentrate in interval $[0.03, 0.07]$.

In addition, we provide some examples of different rarenesses in Table ~\ref{tab:example}. From these examples, we can find that the increase of rareness usually means the complication of caption in three aspects: unseen expression, more thorough description, and action combination. Some words or phrases are uncommon in the training set, such as `x-shape' and `dangling and swinging'. These sentences may contain unseen motions or are hard to understand by the text encoders. An example of an action combination is that 'a person stretches their hips, arms, then bend forwards and steps forwards' contains four unit actions: `stretch hip', `stretch arm', `bend forward', and `step forward'. The generative models are supposed to act them in a row, which is very challenging to current methods. Hence, these examples build up a more difficult and realistic environment for method evaluation.

==> sections/supp_02_results.tex <==
\section{Full Quantitative Comparison}

\begin{table*}[ht]
\centering
\caption{\textbf{Quantitative results on the HumanML3D test set.} For a fair comparison, all methods use the real motion length from the ground truth as the extra given information. `$\uparrow$'(`$\downarrow$') indicates that the values are better if the metric is larger (smaller). We run all the evaluations 20 times. $x^{\pm y}$ indicates that the average metric is $x$ and the the 95\% confidence interval is $y$. The best result and the second best result are in red cells and blue cells, respectively.}
\label{tab:full_humanml3d}
\setlength{\tabcolsep}{1.4mm}
{
\begin{tabular}{lccccccc}
\hline

\multirow{2}{2cm}{\centering Methods} & \multicolumn{3}{c}{\centering R Precision$\uparrow$} & \multirow{2}{1.5cm}{\centering FID$\downarrow$} & \multirow{2}{2.5cm}{\centering MM Dist$\downarrow$} & \multirow{2}{2cm}{\centering Diversity$\uparrow$} & \multirow{2}{2cm}{\centering MultiModality$\uparrow$} \\
& Top 1 & Top 2 & Top 3 \\
\hline
Real motions & $0.511^{\pm .003}$ & $0.703^{\pm.003}$ & $0.797^{\pm.002}$ & $0.002^{\pm.000}$ & $2.974^{\pm.008}$ & $9.503^{\pm.065}$ & -\\ 
\hline

Language2Pose~\cite{ahuja2019language2pose} & $0.246^{\pm.002}$ & $0.387^{\pm.002}$ & $0.486^{\pm.002}$ & $11.02^{\pm.046}$ & $5.296^{\pm.008}$ & $7.676^{\pm.058}$ & - \\

Text2Gesture~\cite{bhattacharya2021text2gestures} & $0.165^{\pm.001}$ & $0.267^{\pm.002}$ & $0.345^{\pm.002}$ & $7.664^{\pm.030}$ & $6.030^{\pm.008}$ & $6.409^{\pm.071}$ & - \\

MoCoGAN~\cite{tulyakov2018mocogan} & $0.037^{\pm.000}$ & $0.072^{\pm.001}$ & $0.106^{\pm.001}$ & $94.41^{\pm.021}$ & $9.643^{\pm.006}$ & $0.462^{\pm.008}$ &
$0.019^{\pm.000}$ \\

Dance2Music~\cite{lee2019dancing} & $0.033^{\pm.000}$ & $0.065^{\pm.001}$ & $0.097^{\pm.001}$ & $66.98^{\pm.016}$ & $8.116^{\pm.006}$ & $0.725^{\pm.011}$ & $0.043^{\pm.001}$ \\

Guo \etal~\cite{guo2022generating}  & $0.457^{\pm.002}$ & $0.639^{\pm.003}$ & $0.740^{\pm.003}$ & $1.067^{\pm.002}$ & $3.340^{\pm.008}$ & $9.188^{\pm.002}$ & \cellcolor{blue!25}$2.090^{\pm.083}$ \\

\hline
MDM~\cite{tevet2022human} & - & - & $0.611^{\pm.007}$ & \cellcolor{blue!25} $0.544^{\pm.044}$ & $5.566^{\pm.027}$ & \cellcolor{red!25} $9.559^{\pm.086}$ & \cellcolor{red!25}$2.799^{\pm.072}$ \\

MotionDiffuse~\cite{zhang2022motiondiffuse} & \cellcolor{red!25} $0.491^{\pm.001}$ & \cellcolor{blue!25} $0.681^{\pm.001}$ & \cellcolor{blue!25} $0.782^{\pm.001}$ & $0.630^{\pm.001}$ & \cellcolor{blue!25} $3.113^{\pm.001}$ & \cellcolor{blue!25} $9.410^{\pm.049}$ &  $1.553^{\pm.042}$ \\
\hline
Ours & \cellcolor{red!25} $0.501^{\pm.005}$ & \cellcolor{red!25} $0.690^{\pm.010}$ & \cellcolor{red!25} $0.787^{\pm.005}$ & \cellcolor{red!25} $0.196^{\pm.006}$ & \cellcolor{red!25} $3.007^{\pm.016}$ & $9.173^{\pm.075}$ & $1.826^{\pm.049}$ \\
\hline
\end{tabular}}
\end{table*}

\begin{table*}[ht]
\centering
\caption{\textbf{Quantitative results on the KIT-ML test set.} $^{\S}$ indicates the results are from our implementation. }
\label{tab:full_kit}
\setlength{\tabcolsep}{1.4mm}
{
\begin{tabular}{lccccccc}
\hline

\multirow{2}{2cm}{\centering Methods} & \multicolumn{3}{c}{\centering R Precision$\uparrow$} & \multirow{2}{1.5cm}{\centering FID$\downarrow$} & \multirow{2}{2.5cm}{\centering MM Dist$\downarrow$} & \multirow{2}{2cm}{\centering Diversity$\uparrow$} & \multirow{2}{2cm}{\centering MultiModality$\uparrow$} \\
& Top 1 & Top 2 & Top 3 \\
\hline
Real motions & $0.424^{\pm .005}$ & $0.649^{\pm.006}$ & $0.779^{\pm.006}$ & $0.031^{\pm.004}$ & $2.788^{\pm.012}$ & $11.08^{\pm.097}$ & -\\ 
\hline

Language2Pose~\cite{ahuja2019language2pose} & $0.221^{\pm.005}$ & $0.373^{\pm.004}$ & $0.483^{\pm.005}$ & $6.545^{\pm.072}$ & $5.147^{\pm.030}$ & $9.073^{\pm.100}$ & - \\

Text2Gesture~\cite{bhattacharya2021text2gestures} & $0.156^{\pm.004}$ & $0.255^{\pm.004}$ & $0.338^{\pm.005}$ & $12.12^{\pm.183}$ & $6.964^{\pm.029}$ & $9.334^{\pm.079}$ & - \\

MoCoGAN~\cite{tulyakov2018mocogan} & $0.022^{\pm.002}$ & $0.042^{\pm.003}$ & $0.063^{\pm.003}$ & $82.69^{\pm.242}$ & $10.47^{\pm.012}$ & $3.091^{\pm.043}$ &
$0.250^{\pm.009}$ \\

Dance2Music~\cite{lee2019dancing} & $0.031^{\pm.002}$ & $0.058^{\pm.002}$ & $0.086^{\pm.003}$ & $115.4^{\pm.240}$ & $10.40^{\pm.016}$ & $0.241^{\pm.004}$ & $0.062^{\pm.002}$ \\

Guo \etal~\cite{guo2022generating}  & $0.370^{\pm.005}$ & $0.569^{\pm.007}$ & $0.693^{\pm.007}$ & $2.770^{\pm.109}$ & $3.401^{\pm.008}$ & $10.91^{\pm.119}$ & \cellcolor{blue!25}$1.482^{\pm.065}$ \\

TEMOS$^{\S}$~\cite{petrovich2022temos} & $0.367^{\pm.005}$ & $0.569^{\pm.004}$ & $0.694^{\pm.006}$ & $2.655^{\pm.051}$ & $3.553^{\pm.016}$ & $9.83^{\pm.081}$ & $0.328^{\pm.015}$ \\
\hline
MDM~\cite{tevet2022human}& -  & - & $0.396^{\pm.004}$ & \cellcolor{blue!25}$0.497^{\pm.021}$ & $9.191^{\pm.022}$ & \cellcolor{blue!25}$10.847^{\pm.109}$ & \cellcolor{red!25}$1.907^{\pm.214}$ \\

MotionDiffuse~\cite{zhang2022motiondiffuse} & \cellcolor{blue!25}$0.417^{\pm.004}$ & \cellcolor{blue!25}$0.621^{\pm.004}$ & \cellcolor{blue!25}$0.739^{\pm.004}$ &  $1.954^{\pm.062}$ &  \cellcolor{blue!25}$2.958^{\pm.005}$ & \cellcolor{red!25} $11.10^{\pm.143}$ & $0.730^{\pm.013}$\\
\hline
Ours & \cellcolor{red!25}$0.427^{\pm.014}$ & \cellcolor{red!25}$0.641^{\pm.004}$ & \cellcolor{red!25}$0.765^{\pm.055}$ & \cellcolor{red!25}$0.155^{\pm.006}$ & \cellcolor{red!25}$2.814^{\pm.012}$ & $10.80^{\pm.105}$ & $1.239^{\pm.028}$ \\
\hline
\end{tabular}}
\end{table*}

Table ~\ref{tab:full_humanml3d} and Table ~\ref{tab:full_kit} show the full comparison between our proposed \name and seven other existing works, including recent diffusion models-based algorithms~\cite{tevet2022human, zhang2022motiondiffuse}. It should be mentioned that the results of Language2Pose~\cite{ahuja2019language2pose}, Text2Gesture~\cite{bhattacharya2021text2gestures}, MoCoGAN~\cite{tulyakov2018mocogan} and Dance2Music~\cite{lee2019dancing} are reported in the paper of HumanML3D dataset~\cite{guo2022generating}. As for TEMOS~\cite{petrovich2022temos}, we modify the official implementation to support the same motion representation as other works and retrain the whole network. Consider that TEMOS does not provide suitable hyper-parameter for the HumanML3D dataset, thus we only report the evaluation results on the KIT-ML dataset. Other results are directly included in the corresponding papers.

Compared to other diffusion model-based pipelines, our proposed \name achieve a better balance between the condition-consistency and fidelity. It should be noted that, \name is the first work to achieve state-of-the-art on both metrics, which demonstrates the superiority of the proposed pipeline. 

% \subsection{Qualitative Results}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/vis1.pdf}
%     \caption{\textbf{Visualization of \name}}
%     \label{fig:vis_ours}
% \end{figure*}

==> sections/supp_03_pose.tex <==
\section{Exploration on Pose Retrieval}

Inspired by AvatarCLIP~\cite{hong2022avatarclip}, we aim to retrieve a relevant pose based on the user input and use these retrieved poses to enhance the motion generation results. The following subsections briefly introduce the pose retrieval technique used in the AvatarCLIP. Then we will illustrate how to incorporate these candidate poses into the motion generation pipeline.

\subsection{Pose Retrieval}

As shown in Figure ~\ref{fig:pipeline_clip}, we get poses from the amass dataset to form a large-scale codebook containing millions of pose data. To better reduce the size, we first use VPoser to encode each pose into a 32-d dimensionality and use K-means clustering to get 1024 cluster centroids. For each cluster centroid, we acquired the original pose parameter by using the VPoser decoder. Rendered from different views, we get a series of pictures of a single 3D gesture. CLIP~\cite{radford2021learning} is applied here to get visual features. During the training period and inference time, we retrieve $k$-th most similar poses from the database by calculating the similarity between the text and visual features. These poses will be sent to the cross-attention module to enhance the motion generation process.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/modified_attention.png}
    \caption{\textbf{The structure of Modified Semantic-Modulated Attention.}}
    \label{fig:modified_attention}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/pose_retrieval.png}
    \caption{\textbf{Pose Retrieval Pipeline in AvatarCLIP~\cite{hong2022avatarclip}}}
    \label{fig:pipeline_clip}
\end{figure}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/vis2.pdf}
    \caption{\textbf{Visualization of Pose-enhanced \name}}
    \label{fig:vis_pose}
\end{figure*}


\subsection{Modified Semantics-Modulated Attention}





Unlike retrieved motion sequences, here we select the top 2 poses and embed the pose parameters into feature vectors. These vectors are directly used to refine motion sequences as shown in Figure ~\ref{fig:modified_attention}. Other settings remain unchanged.

\subsection{Experimental Results}

\begin{table}[t]
\centering
\caption{\textbf{Quantitative results of pose retrieval on KIT testset.}}
\label{tab:pose}
\setlength{\tabcolsep}{1.4mm}
{
\begin{tabular}{ccc}
\hline

Method & Top 1$\uparrow$ & FID$\downarrow$ \\
\hline
Baseline & $0.421^{\pm.012}$ & $0.245^{\pm.008}$ \\
Pose Retrieval & $0.422^{\pm.012}$ & $0.251^{\pm.009}$ \\
\hline
\end{tabular}}
\vspace{-10pt}
\end{table}


This section provides some preliminary evaluation of the pose retrieval technique. As shown in Table ~\ref{tab:pose}, the quantitative results are almost the same when we use selected poses to enhance the motion generation process. However, we find some other interesting uses of this technique. Figure ~\ref{fig:vis_pose} shows the generated motion sequences with two different given text descriptions. The only difference between them is that we describe the body shape in the second one. It should be mentioned that, in the KIT-ML dataset, we use 3D key points as the primary motion representation. The visualized meshes are generated from SMPLify~\cite{bogo2016keep}. The visual feature of our retrieved poses may be consistent with the description "tall", thereby guiding the denoising steps to synthesize a motion sequence with a tall skeleton. 

This technique may be further explored and can be a significant supplementary to our \name, enhancing the consistency between visual description and the synthesized motion sequences. 
